Using Process Calculus for Optimizing Data and Computation Sharing in Complex Stateful Parallel Computations

We propose novel techniques that exploit data and computation sharing to improve the performance of complex stateful parallel computations, like agent-based simulations. Parallel computations are translated into behavioral equations, a novel formalism layered on top of the foundational process calculus $\pi$-calculus. Behavioral equations blend code and data, allowing a system to easily compose and transform parallel programs into specialized programs. We show how optimizations like merging programs, synthesizing efficient message data structures, eliminating local messaging, rewriting communication instructions into local computations, and {aggregation pushdown} can be expressed as transformations of behavioral equations. We have also built a system called OptiFusion that implements behavioral equations and the aforementioned optimizations. Our experiments showed that OptiFusion is over 10$\times$ faster than state-of-the-art stateful systems benchmarked via complex stateful workloads. Generating specialized instructions that are impractical to write by hand allows OptiFusion to outperform even the hand-optimized implementations by up to 2$\times$.

==> preamble-comments.tex <==
\usepackage[inline]{enumitem}
\usetikzlibrary{shapes,positioning}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % FIXME: Remove for submission - changes to page margins to enable margin comments
 \paperwidth=\dimexpr \paperwidth + 8cm\relax
 \oddsidemargin=\dimexpr\oddsidemargin + 4cm\relax
 \evensidemargin=\dimexpr\evensidemargin + 4cm\relax
 \marginparwidth=\dimexpr \marginparwidth + 5cm\relax
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % FIXME: Todonotes inclusion
\usepackage[textwidth=4cm,textsize=footnotesize]{todonotes}% Package inclusion
\makeatletter
\tikzstyle{notestyleraw} = [
    draw = none,%\@todonotes@currentbordercolor, 
    fill = \@todonotes@currentbackgroundcolor,
    text = \@todonotes@currenttextcolor,
    line width = 1pt,
    text width = \@todonotes@textwidth - 1.6 ex - 2pt, 
    inner sep = 0.8 ex,
    xshift=2.8cm
    ]
\makeatother
% % Define author colors for todonotes
\def\ztcolor{blue}  
% Define author names for todonotes
\def\ztname{Zilu}

\newcommand{\changem}[1]{\textcolor{purple}{#1}}
\newcommand{\changea}[1]{\textcolor{red}{#1}}
\newcommand{\changeb}[1]{\textcolor{blue}{#1}}
\newcommand{\changec}[1]{\textcolor{orange}{#1}}

\def\dancolor{orange}
\def\danname{Dan}
% % Set up todonotes author versions
 \newcommand*{\commonsetup}{\setlist[itemize]{align=parleft,left=0pt..1em}\setlist[enumerate]{align=parleft,left=0pt..1em}}
 \newcommand*{\setupzt}{\commonsetup\setuptodonotes{color=\ztcolor,textcolor=white,caption={}}}
\newcommand*{\setupdan}{\commonsetup\setuptodonotes{color=\dancolor,textcolor=white,caption={}}}

% % Set up todonotes author specific commands
 \makeatletter
 \newcommand{\zt} [2][\@nil]{\bgroup\setupzt\todo[inline]{\sffamily\textbf{\ztname\def\tmp{#1}\ifx\tmp\@nnil\else~[#1]\fi:~}#2}\egroup}
 \newcommand{\mzt}[2][\@nil]{\bgroup\setupzt\todo        {\sffamily\textbf{\ztname\def\tmp{#1}\ifx\tmp\@nnil\else~[#1]\fi:~}#2}\egroup}
 \newcommand{\dan}[2][\@nil]{\bgroup\setupdan\todo        {\sffamily\textbf{\danname\def\tmp{#1}\ifx\tmp\@nnil\else~[#1]\fi:~}#2}\egroup}
 \makeatother
% % FIXME: End of todonotes inclusion
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> sec-background.tex <==
\section{Background}
\label{sec:background}

% Vertex-centric programming {was} first proposed and popularized by Google's Pregel \cite{pregel} for the efficient processing of large distributed graphs. Later other frameworks like GraphX \cite{graphx13} and Flink \cite{flink-pregel} have also supported this paradigm for parallel graph processing, implementing the vertex-centric paradigm via a Pregel-like operator. Though there are differences among such frameworks concerning details such as whether the graph topology and vertex state are mutable, all these frameworks share the same assumption as Pregel, where vertices interpret the same user-defined function iteratively in every superstep.

% Giraph \cite{facebook-giraph} is an open-source implementation of Pregel and has also been widely adopted in the industry. 

% Graph-centric programming was proposed by Giraph++ \cite{TianBCTM13}, which aims to address the inefficiency of processing 

% In this section, we use Pregel as an example and explain its syntax and semantics to familiarize users with vertex-centric programming. More concretely, we show how to implement a classic graph algorithm, PageRank \cite{PageRank}, which represents the target applications that Pregel is designed for. We also explain what agent-based simulations are and how they can be expressed as complex vertex programs. 

\subsection{Vertex-Centric Paradigm}
\subsubsection{Giraph syntax}
Giraph~\cite{facebook-giraph} is an open-source implementation of Pregel~\cite{pregel}. For demonstration, we present Giraph syntax using Scala pseudocode in \cref{code:vertex-api}. Each vertex has a unique id and can obtain the current superstep (line 2). Users need to define $\syntax{compute}$ (line 8), which specifies the behavior of a vertex that is executed in each superstep, such as updating local states (lines 3--4), processing messages (line 6), and sending messages to neighbors (lines 5, 9). If there is no further work until new messages arrive, a vertex votes to halt (line 10).
\begin{figure}
    \centering
\begin{code}
abstract class Vertex[VertexId, VertexValue, EdgeValue, MessageValue] {
    def superstep(): Int = 0
    def getVertexValue(): VertexValue
    def setVertexValue(v: VertexValue): Unit
    def iterator(): Iterator[VertexId]
    def getMessages(): Iterator[MessageValue]
    def getNumOutEdges(): Int
    def compute(msgs: Iterator[MessageValue]): Unit 
    def sendMessageTo(dest: VertexId, message: MessageValue): Unit
    def voteToHalt(): Unit
}
\end{code}
\Description{An API that illustrates core instructions in Giraph DSL}
    \caption{Core Giraph DSL.}
    \label{code:vertex-api}
\end{figure}

Users define a vertex program by creating a subclass that extends the $\syntax{Vertex}$ class. In particular, users provide types for $\syntax{VertexId}$, $\syntax{VertexValue}$, $\syntax{EdgeValue}$, and $\syntax{MessageValue}$ (line 1) and override the $\syntax{compute}$ method (line {8}) with vertex behavior. All vertices in a graph execute the same $\syntax{compute}$ method concurrently.

\subsubsection{Computational model}
The computational model of Giraph~\cite{pregel, facebook-giraph} closely follows the BSP processing model~\cite{valiant90BSP}, which is an abstract parallel machine that is commonly used by distributed frameworks for parallel computing. This abstract machine contains:
\begin{itemize}
    \item a set of processors. Each processor can be viewed as a core-memory pair, where the memory is private to the core. A core can perform arbitrary computations over values stored in its memory. Processors communicate by sending messages, which arrive at the beginning of a superstep; 
    \item a synchronization facility to synchronize all processors periodically.
\end{itemize}
Computations on a BSP machine proceed in a sequence of superstep, separated by global synchronization. Per superstep, a processor performs local updates, processes received messages, and generates messages for other processors. A superstep consists of a sequence of local steps. Messages are sent at the end of a superstep and arrive in the next superstep.

A Giraph program has two inputs, an input graph and a vertex program to be executed by each node in the graph. Every vertex can be regarded as a BSP processor. Computations proceed iteratively.
Initially, all vertices are \emph{active}. In each superstep, every active vertex executes its $\syntax{compute}$ method in parallel. A superstep ends when all active vertices have completed executing $\syntax{compute}$. An active vertex becomes \emph{inactive} by voting to halt (through the instruction $\syntax{voteToHalt}$), suggesting that it has no more work to do until new messages arrive. An inactive vertex becomes active if it has received at least one message at the beginning of a superstep, and remains inactive otherwise. Messages are sent at the end of a superstep and are available for processing at the beginning of the next superstep. A program terminates when all vertices have become \emph{inactive} and there is no more message in the system. 

\subsubsection{Example}
% the accumulative iterative update
We adapt the PageRank example presented in \cite{TianBCTM13} as our running example, to illustrate the difference between vertex-centric and graph-centric implementations. 
% , we also consider an  variant of the PageRank algorithm that updates accumulative values asynchronously \cite{zhang2012accelerate}, which is shown to converge to the same value as the classic PageRank \cite{PageRank}. 
% Asynchronous Accumulative Updates

\begin{example}[PageRank]
\label{ex:pageRank}
The PageRank algorithm computes the importance of web pages based on the assumption that a page is more important if it receives links from other important pages~\cite{PageRank}. Each page has a PageRank value, where a higher value suggests that a page is more important. PageRank also introduces a damping factor to model the probability of a user continuing to click on links instead of jumping to a random page, typically set to 0.85. The damping factor adjusts the distribution of a page's PageRank during the iterative update. 

The classic PageRank algorithm is synchronous and proceeds in the following two phases:
\begin{itemize}
    \item Initialization: Assign an initial PageRank value to each page in the system. Initially, all pages have equal PageRank values;
    \item {Iterative Update:
        \begin{itemize}
            \item For each page, calculate its new PageRank value based on the incoming links from other pages.
            \item Distribute a fraction of the current page's PageRank to the pages it links to. The amount distributed is proportional to the current page's PageRank and inversely proportional to the number of its outgoing links.
            \item Update the PageRank values for all pages.
        \end{itemize}}
        Repeat the above steps until the PageRank values converge (no significant changes).
\end{itemize}

The classic PageRank algorithm is easy to understand and straightforward to implement on a synchronous BSP system. In~\cite{TianBCTM13}, authors considered a variant of the PageRank algorithm with accumulative intermediate updates as described in~\cite{zhang2012accelerate}. As the name suggests, this variant accumulates the intermediate update results in a $\syntax{delta}$ variable in each vertex, instead of modifying the PageRank value of a vertex. This version of the PageRank algorithm has been shown to converge much faster than the classic PageRank algorithm while converging to the same value.
\end{example}

The implementation of the PageRank algorithm with accumulative intermediate updates in Giraph is shown in \cref{code:pagerank-pregel} (adapted from \cite{TianBCTM13}). Each vertex has a local state that denotes its accumulated intermediate updates in the current superstep (line 4). In superstep 0, the PageRank value of each vertex is initialized to 0.15 (lines 5--8). Per superstep, a vertex processes received messages, computes the accumulated intermediate updates, and sends messages to neighbors (lines 9--13). 

\begin{figure}
    \centering
\begin{code}
class PageRankVertex extends Vertex[Long, Double, Unit, Double] {
    override def compute(msgs: Iterator[Double]): Unit = {
        if (superstep() <= MAX_ITERATION){
            var delta: Double = 0
            if (superstep() == 0) {
                setVertexValue(0)
                delta += 0.15
            }
            delta += sum(msgs)
            if (delta > 0) {
                setVertexValue(getVertexValue() + delta)
                sendMessageToAllEdges(0.85*delta / getNumOutEdges())
            }
        }
        voteToHalt()
    }
}
\end{code}
\Description{Pseudocode that implements the asynchronous PageRank example in Giraph}
\caption{PageRank implementation in Giraph.}
\label{code:pagerank-pregel}
\end{figure}

\subsection{Graph-Centric Paradigm}
\paragraph{Giraph++ syntax}
Giraph++ generalizes the vertex-centric programming model to the graph-centric paradigm~\cite{TianBCTM13}. We summarize the core syntax of Giraph++ using Scala pseudocode in \cref{code:graph-api}. The core abstraction in Giraph++ is $\syntax{GraphPartition}$. 

Similar to Giraph, users define a graph-centric program by creating a subclass that extends the $\syntax{GraphPartition}$ class, providing type variables for $\syntax{VertexId}$, $\syntax{VertexValue}$, $\syntax{EdgeValue}$, and $\syntax{MessageValue}$ (line 1). Many methods in $\syntax{GraphPartition}$ (lines 2, 11 -- 13) are similar to that of \cref{code:vertex-api}. Just like a $\syntax{Vertex}$ program, a $\syntax{GraphPartition}$ program needs to contain a $\syntax{compute}$ method (line {11}) that specifies the behavior of vertices in a graph partition. 
Compared with $\syntax{Vertex}$, $\syntax{GraphPartition}$ introduces the following main differences:
\begin{itemize}
    \item methods for querying and updating vertices in a partition (lines 3, 6, 10); 
    \item methods for distinguishing \emph{internal} and \emph{boundary} vertices in a partition (lines 4--5), explained shortly; and 
    \item methods for programming distinct behaviors for internal and boundary vertices in a partition (lines 7--9).
\end{itemize}
The $\syntax{GraphPartition}$ abstraction makes data placement explicit at the partition level: a vertex can distinguish whether a neighbor vertex is remote or local. This enables data and computation sharing among local vertices in a partition. Messages are only sent between boundary vertices, while communication among internal vertices is through local data sharing. 

\begin{figure}
    \centering
\begin{code}
abstract class GraphPartition[VertexId, VertexValue, EdgeValue, MessageValue] {    
    def superstep: Int = 0
    def containsVertex(id: VertexId): Boolean
    def isInternalVertex(id: VertexId): Boolean
    def isBoundaryVertex(id: VertexId): Boolean
    def getVertex(id: VertexId): Vertex[VertexId, VertexValue, EdgeValue, MessageValue]
    def internalVertices(): Set[Vertex[VertexId, VertexValue, EdgeValue, MessageValue]]
    def activeInternalVertices(): Set[Vertex[VertexId, VertexValue, EdgeValue, MessageValue]]
    def boundaryVertices(): Set[Vertex[VertexId, VertexValue, EdgeValue, MessageValue]]
    def allVertices(): Set[Vertex[VertexId, VertexValue, EdgeValue, MessageValue]]
    def compute(msgs: Iterator[MessageValue]): Unit 
    def sendMessageTo(dest: VertexId, message: MessageValue): Unit
    def allVoteToHalt(): Unit
}
\end{code}
\Description{An API that illustrates core instructions in Giraph++ DSL}
    \caption{Core Giraph++ DSL.}
    \label{code:graph-api}
\end{figure}

\paragraph{Computational model}
The computational model of Giraph++ follows the BSP model, just like Giraph. The main difference is the granularity of computations: per superstep, computations are applied to parallel graph partitions instead of parallel vertices. A superstep executed by a graph partition is applied to all vertices in the partition. The $\syntax{voteToHalt}$ instruction in \cref{code:vertex-api} has been changed to $\syntax{allVoteToHalt}$ in \cref{code:graph-api}, suggesting all internal vertices in a graph partition have voted to halt.

As we have seen, Giraph++ distinguishes between \emph{internal} and \emph{boundary} vertices. 
Internal vertices in a graph partition are just like ordinary vertices in Giraph. Such a vertex has two states, active and inactive, and a graph has all the information about it, including vertex value, edge values, and received messages. A vertex is internal only to one partition, which is also called \emph{owner}. 

Boundary vertices can be duplicated in zero or more copies across partitions. The \emph{primary copy} of a boundary vertex is the corresponding internal vertex that resides in its owner partition. 
A partition only has information about the vertex value of a boundary vertex, which is a \emph{cached copy} of the vertex value of the primary copy. Different copies of boundary vertices are synchronized through messages with their primary copies to remain consistent.


\subsubsection{Example}
We revisit the PageRank algorithm with accumulative iterative updates explained in~\cref{ex:pageRank}. Here we express the algorithm using the $\syntax{GraphPartition}$ abstraction, shown in \cref{code:pagerank-giraph++}. 

\begin{figure}[h]
    \centering
\begin{code}
class PageRankPartition extends GraphPartition[VertexId, Double, Unit, Double] {
    override def compute(msgs: Iterator[Double]): Unit = {
        if (superstep() <= MAX_ITERATION){
            if (superstep() == 0) {
                allVertices().foreach(v => {
                    v.getVertexValue().pr = 0
                    v.getVertexValue().delta = 0
                })
            }
            activeInternalVertices().foreach(v => {
                if (superstep() == 0) {
                    v.getVertexValue().delta += 0.15
                }
                v.getVertexValue().delta += sum(v.getMessages())
                if (v.getVertexValue().delta > 0) {
                    v.getVertexValue().pr += v.getVertexValue().delta
                    update = 0.85*v.getVertexValue().delta / v.getNumOutEdges()

                    while (v.iterator().next) {
                        neighbor = getVertex(v.iterator().next)
                        neighbor.getVertexValue().delta += update
                    }
                }
                v.getVertexValue().delta = 0
            })
            boundaryVertices().foreach(v => {
                if (v.getVertexValue().delta > 0) {
                    sendMessageTo(v.getVertexId(), v.getVertexValue().delta)
                    v.getVertexValue().delta = 0
                }    
            })
            allVoteToHalt()
        }
    }
}
\end{code}    
\Description{Pseudocode that implements the asynchronous PageRank example in Giraph++}
\caption{PageRank implementation in Giraph++.}
\label{code:pagerank-giraph++}
\end{figure}

% Every vertex in a partition has two attributes, a page rank value ($\syntax{pr}$) and an accumulated intermediate updates ($\syntax{delta}$) (lines 6--7), initially 0. 
Users express separate behavior for internal (lines 10--25) and boundary vertices (lines 26--31). For internal vertices, communication is through local data sharing (lines 19--22) and updates are applied immediately. For boundary vertices, communication is through sending messages (line 28).

\paragraph{Local asynchrony}
An important assumption that underlies the graph-centric paradigm in Giraph++ is leveraging local asynchrony in iterative algorithms for better performance~\cite{zhang2012accelerate}. Local asynchrony allows asynchronous computations among internal vertices in a partition: vertices can immediately observe the latest value of other internal vertices within the same superstep. This is evident in the PageRank implementation in \cref{code:pagerank-giraph++}, where the value of vertices are updated in-place (lines 14, 16) and immediately observed and modified by other internal vertices (lines 20--21).

While local asynchrony enables faster convergence, this assumption limits the applicability of the graph-centric approach. More importantly, this suggests that the semantics of a vertex-centric program is not preserved if simply compiling messages away into local computation.

\paragraph{Data and computation sharing}
While exploiting local asynchrony leads to faster convergence hence fewer iterations, graph-centric paradigm also harnesses data and computation sharing to reduce time per iteration. This can also be seen in \cref{code:pagerank-giraph++}. On line 17, common computations are factored out and materialized as the value of $\syntax{update}$, which is then shared among vertices (line 21). Vertices also use data sharing to communicate locally (lines 19--22).

% \subsection{Partial Evaluation and Multi-stage Programming}
% Multi-stage programming is commonly used to bridge the gap between high-level expressiveness and low-level efficiency. The classic example that illustrates the motivation for multi-stage programming is the generic power function $\syntax{power}(x, n)$ \cite{Taha03}: 
% \begin{code}
% def power(x: Int, n: Int): Int = {
%     if (n==0) 
%         1  
%     else  
%         x * power(x, n-1) 
% }
% \end{code}
% This high-level generic function provides a nice abstraction that makes defining other special functions straightforward:
% \begin{code}
% def square(x: Int): Int = power(x, 2)
% def cube(x: Int): Int = power(x, 3)
% \end{code}

% However, this abstraction comes at the cost of performance. In particular, a low-level implementation of $\syntax{square}$ that multiplies $x$ with itself will be faster than invoking $\syntax{power}$, which computes the result recursively. Not all hope is lost though. On line 1, the body of $\syntax{square}$ has a constant argument 2 that is known statically. Therefore, we can apply staging to rewrite the body of $\syntax{square}$ with the partially evaluated program generated from $\syntax{power}(x, 2)$, making it possible to achieve both the high-level programming abstractions and the high-performance of low-level implementations.

% % We note that staging is a standard technique used to address sources of program inefficiency like dispatching overhead, and is commonly used in areas such as designing domain-specific languages (DSL) \cite{SheardBP99, HerrmannL06, Jetbrain, Forge13, AxelssonCDHKLPSSV10, DeVitoHAHV13, LeeBSCROO11, RompfO10} and constructing compilers to generate more efficient code \cite{Ulrik86, RompfSABJLJOO13, RompfSBLCO14, PuschelMJPVSXFG05, OfenbeckRSOP13}. 

% The parallelism between how staging is applied in the classic $\syntax{power}$ example and our work is clear: we similarly exploit the fact that when dispatching on the value of supersteps in vertex programs, the value of supersteps in the conditions are often known statically, which allows us to avoid such overhead by rewriting the original program with more efficient instructions that only compute useful code via staging. 

% \begin{code}
% def vertex(): Unit
% def vertex(g: Graph): Graph
% def partition() = vertex(partition1)
% \end{code}
